An homotopy method for $\ell_p$ regression provably beyond self-concordance and in input-sparsity time

We consider the problem of linear regression where the $\ell_2^n$ norm loss (i.e., the usual least squares loss) is replaced by the $\ell_p^n$ norm. We show how to solve such problems up to machine precision in $O^*(n^{|1/2 - 1/p|})$ (dense) matrix-vector products and $O^*(1)$ matrix inversions, or alternatively in $O^*(n^{|1/2 - 1/p|})$ calls to a (sparse) linear system solver. This improves the state of the art for any $p\not\in \{1,2,+\infty\}$. Furthermore we also propose a randomized algorithm solving such problems in {\em input sparsity time}, i.e., $O^*(Z + \mathrm{poly}(d))$ where $Z$ is the size of the input and $d$ is the number of variables. Such a result was only known for $p=2$. Finally we prove that these results lie outside the scope of the Nesterov-Nemirovski's theory of interior point methods by showing that any symmetric self-concordant barrier on the $\ell_p^n$ unit ball has self-concordance parameter $\tilde{\Omega}(n)$.

==> intro_old.tex <==

\section{Introduction}
Linear programming is concerned with optimization problems of the form:
$$\min_{x \in \R^d_+ : \ A x = b} c \cdot x ~,$$
for some $A \in \R^{n \times d}, b \in \R^n, c \in \R^d$. In practice such problem often comes with a guarantee on how far a solution can be, in which case the problem can be rewritten as (up to rescaling)
$$\min_{x \in \R^d : \ \|x\|_{\infty} \leq 1 \ \text{and} \ A x = b} c \cdot x ~.$$
Classical interior point methods theory show that such problems can be solved up to machine precision in roughly $\sqrt{n}$ calls to a $d \times d$ linear system solver, see e.g., \cite{NN94}. State of the art results by \cite{LS14} show that in fact (up to logarithmic factors) $\sqrt{n}$ can be replaced by $\sqrt{d}$. Furthermore this number of iterations is {\em optimal} in the Nesterov-Nemirovski's theory of interior point methods in the sense that {\em any} self-concordant barrier on the hypercube $\{x \in \R^d : \|x\|_{\infty} \leq 1\}$ has self-concordance parameter $\nu \geq d$ (recall that the square root of the self-concordance parameter controls the number of iterations for interior point methods).
%that an $\epsilon$-approximate solution for this problem can be obtained in roughly $\sqrt{d} \log(1/\epsilon)$ iterations of {\em interior point methods}, where each iteration is roughly of the same order of complexity (or even possibly smaller) as solving a linear system. 
\newline

%for the original formulation, perhaps formulate the AGD result rather than SVRG because it's better for the subproblems.

In this paper we investigate the complexity of replacing the $\ell_{\infty}$ constraint by an $\ell_p$ constraint, $1<p<+\infty$, that is:
\begin{equation} \label{eq:classicalformulation} 
\min_{x \in \R^d : \ \|x\|_{p} \leq 1 \ \text{and} \ A x = b} c \cdot x ~.
\end{equation}
Clearly the case of $\ell_2$ exactly corresponds to solving a linear system. Moreover it is well-known that for the Euclidean ball $\{x : \|x\|_2 \leq 1\}$ there exists a barrier with self-concordance parameter $\nu=1$, and thus the Nesterov-Nemirovski's interior point methods theory correctly predicts that the case $p=2$ can be solved in a dimension-free number of iterations. Our contribution is to show that the Nesterov-Nemirovski theory is provably suboptimal for any $p \not\in \{1,2,\infty\}$. More precisely we show that for any $p \neq 2$, any {\em symmetric} self-concordant barrier on $\{x \in \R^d : \|x\|_p \leq 1\}$ has self-concordance parameter $\tilde{\Omega}_p(d)$. On the other hand we propose a new homotopy method which requires only $\tilde{O}_p(n^{|1/2 - 1/p|})$ iterations\footnote{We use the notation $O_p$ to hide polynomial factors in $p/(p-1)$.}\footnote{We note that the dual problem to \eqref{eq:classicalformulation} corresponds to the $\ell_q$ norm problem (where $1/p+1/q=1$) but we shall not use this fact and we treat any $p \in (1,+\infty)$ (observe that $|1/2-1/p|=|1/2-1/q|$).}, thus interpolating between the known results for $p \in \{1,2,+\infty\}$. Slightly more precisely our homotopy method runs in $\tilde{O}_p(n^{|1/2 - 1/p|})$ calls to a sparse linear system solver (if $A$ is sparse), or alternatively in $\tilde{O}_p(n^{|1/2 - 1/p|})$ dense matrix-vector products and $\tilde{O}_p(1)$ matrix inversions. We note that there is no known algorithm for $p=\infty$ (i.e., for linear programming) with the latter running time, and such a result would in our opinion be a major breakthrough. Unfortunately our approach does not {\em a priori} shed light on this problem since our running time explodes as $p$ tends to infinity or $1$.
%(where each iteration amounts to solving a few linear systems).
\newline

In the rest of the paper we consider the following problem, which we refer to as $\ell_p$ regression:
\begin{equation} \label{eq:regressionformulation}
\min_{x \in \R^d} c \cdot x + \|A x - b\|_p^p ~.
\end{equation}
Observe that to have a bounded solution we need to assume that $c \in \mathrm{ker}(A)^{\perp}$. Note also that \eqref{eq:classicalformulation} can essentially be reduced to \eqref{eq:regressionformulation} by using the matrix $\left( {\begin{array}{cc}
   \lambda A & 0 \\
   0 & \mu I_d \\
  \end{array} } \right)$ and target vector $\left( {\begin{array}{cc}
   \lambda b \\
   0 \\
  \end{array} } \right)$ for some $\lambda>0$ large enough and some $\mu>0$.
\newline

In Section \ref{sec:hom} we give our new homotopy method to solve \eqref{eq:regressionformulation}. In Section \ref{sec:inputsparsity} we show how to combine this new method with recent advances in accelerated stochastic gradient descent to obtain an algorithm running in input sparsity time. Finally in Section \ref{sec:lb} we prove the $\tilde{\Omega}(n)$ lower bound on the self-concordance parameter for barriers on the $\ell_p^n$ ball.
%
%\begin{remark} \label{rmk:nologs}
%In order to focus the discussion on our main new arguments we ignore floating point errors in this paper. In particular, for methods reaching an $\epsilon$-optimal point in $K \log(1/\epsilon)$ iterations, we will simply say that the method reaches an optimal point in $O(K)$ iterations. We note however that our algorithms are robust in the sense that all the logarithmic terms could be made explicit at the expense of making the proofs more technical.
%\end{remark}
